A Syntactic Approach to Studying Strongly Equivalent Logic Programs

In the field of Answer Set Programming (ASP), two logic programs are strongly equivalent if they are ordinarily equivalent under any extensions. This property provides a theoretical foundation for studying many aspects of logic programs such as program simplification and transformation etc. Therefore, strong equivalence has been investigated extensively for ASP and its extensions such as LPMLN. In this paper, we present a syntactic approach to studying the strong equivalence of logic programs, which provides several interesting results and would help us understand the strong equivalence from a new perspective. Firstly, we present the notions of independent sets and five kinds of syntactic transformations (S-* transformations) for logic programs. And we investigate the strong equivalence (SE) and non-strong equivalence (NSE) preserving properties of the S-* transformations in the contexts of ASP and LPMLN. Secondly, based on the properties of the S-* transformations, we present a fully automatic algorithm to discover syntactic conditions that preserve strong equivalences (SE-conditions) of ASP and LPMLN programs. To discover the SE-conditions efficiently, we present four kinds of approaches to improve the algorithm. Thirdly, we present a preliminary method to simplify the discovered SE-conditions and report the simplified SE-conditions of several kinds of LPMLN programs. After that, we present a discussion on the discovered SE-conditions and some existing problems. Finally, we present a comparison between SE-conditions discovering approaches in this paper and in the related work.

==> acknowledgement.tex <==
%!TEX root = lpmln_isets.tex


\section{Acknowledgements}
We are grateful to the anonymous referees for their useful comments on the earlier version of this paper. 
The work was supported by the National Key Research and Development Plan of China (Grant No.2017YFB1002801).


==> s_ad_sat_table.tex <==
%!TEX root = lpmln_isets.tex


\begin{table}
    \centering
    \caption{Satisfiability between HT-interpretations and \lpmln rules under the S-AD Transformation}
    \label{tab:single-add-sat}
    \begin{threeparttable}
    \begin{tabular}{lccc}
        \hline
        $\#$ & Rule Types & $(X, Y) \models r$ & $(X, Y) \not\models r$  \\
        \hline
        1. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$
            & $(X', Y') ~\models~  \sadd{r}$ & $(X', Y') ~\not\models~  \sadd{r}$\\\hline

        \multirow{3}{*}{2.} & \multirow{3}{*}{$\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$} 
            & $(X, Y) ~\models~  \sadd{r}$ & $(X, Y) ~\not\models~  \sadd{r}$ \\   
            &   & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ or ${\seinthalfadd{X}{Y} ~\not\models~  \sadd{r}}$ & $\seinthalfadd{X}{Y} ~\not\models~  \sadd{r}$\\
            &   & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$ \\ \hline

        \multirow{3}{*}{3.} & \multirow{3}{*}{$\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$} 
            & \multirow{3}{*}{$(X', Y') \models \sadd{r}$} & ${(X, Y) ~\models~  \sadd{r}}$\\ 
            &  &  & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
            &  &   & $\seintadd{X}{Y} ~\not\models~  \sadd{r}$ \\ \hline

        \multirow{3}{*}{4.} & \multirow{3}{*}{$\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$} 
            & \multirow{3}{*}{$(X', Y') \models \sadd{r}$} & $(X, Y) ~\not\models~  \sadd{r}$\\ 
            &  &  & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
            &  &  & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$ \\ \hline

        \multirow{3}{*}{5.} & \multirow{3}{*}{$\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$} 
             & \multirow{3}{*}{$(X', Y') \models \sadd{r}$} & $(X, Y) ~\not\models~  \sadd{r}$\\ 
            &   &  & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
            &  &   & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$  \\ \hline

            6. & Others & $(X', Y') \models \sadd{r}$ & \textemdash\\ 
        \hline
        \end{tabular}

        \begin{tablenotes}
            \item $(X', Y') \in \{(X, Y), \seinthalfadd{X}{Y}, \seintadd{X}{Y}\}$. 
        \end{tablenotes}
    \end{threeparttable}
\end{table}


% \begin{table}
%     \centering
%     \caption{Satisfiability between SE-interpretations and rules w.r.t. the Single Addition}
%     \label{tab:single-add-sat}
%     \begin{threeparttable}
%     \begin{tabular}{lccc}
%         \hline
%         $\#$ & Case & $(X, Y) \models r$ & $(X, Y) \not\models r$  \\
%         \hline
%         \multirow{3}{*}{1.} & \multirow{3}{*}{$\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$} 
%             & $(X, Y) ~\models~  \sadd{r}$ & $(X, Y) ~\not\models~  \sadd{r}$\\ 
%             &  & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ & $\seinthalfadd{X}{Y} ~\not\models~  \sadd{r}$\\
%             &   & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & $\seintadd{X}{Y} ~\not\models~  \sadd{r}$ \\ \hline

%         \multirow{3}{*}{2.} & \multirow{3}{*}{$\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$} 
%             & $(X, Y) ~\models~  \sadd{r}$ & $(X, Y) ~\not\models~  \sadd{r}$ \\   
%             &   & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ or ${\seinthalfadd{X}{Y} ~\not\models~  \sadd{r}}$ & $\seinthalfadd{X}{Y} ~\not\models~  \sadd{r}$\\
%             &   & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$ \\ \hline

%         \multirow{3}{*}{3.} & \multirow{3}{*}{$\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$} 
%             & $(X, Y) ~\models~  \sadd{r}$ & ${(X, Y) ~\models~  \sadd{r}}$\\ 
%             &  & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
%             &  & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & $\seintadd{X}{Y} ~\not\models~  \sadd{r}$ \\ \hline

%         \multirow{3}{*}{4.} & \multirow{3}{*}{$\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$} 
%             & $(X, Y) ~\models~  \sadd{r}$ & $(X, Y) ~\not\models~  \sadd{r}$\\ 
%             &  & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
%             &  & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$ \\ \hline

%         \multirow{3}{*}{5.} & \multirow{3}{*}{$\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$} 
%              & $(X, Y) ~\models~  \sadd{r}$ & $(X, Y) ~\not\models~  \sadd{r}$\\ 
%             &   & $\seinthalfadd{X}{Y} ~\models~  \sadd{r}$ & ${\seinthalfadd{X}{Y} ~\models~  \sadd{r}}$\\
%             &  & $\seintadd{X}{Y} ~\models~  \sadd{r}$  & ${\seintadd{X}{Y} ~\models~  \sadd{r}}$  \\ \hline

%             \multirow{2}{*}{6.} & \multirow{2}{*}{Others} & $(X, Y) \models \sadd{r}$, $\seinthalfadd{X}{Y} \models \sadd{r}$, & \multirow{2}{*}{\textemdash}\\ 
%              & &  and $\seintadd{X}{Y} \models \sadd{r}$ & \\ 
%         \hline
%         \end{tabular}

%         \begin{tablenotes}
%             \item[*] $(X', Y') \in \{(X, Y), \seinthalfadd{X}{Y}, \seintadd{X}{Y}\}$. 
%             \item[*] In Case 2, if $(X, Y) \models r$ and $\seinthalfadd{X}{Y} \not\models \sadd{r}$, we have $Y \not\models r$ and $X \not\models r$, i.e. $\hr{r} \cap Y = \emptyset$, $\pbr{r} \subseteq X \subseteq Y$, $\nbr{r} \cap Y = \emptyset$, which means $I \cap Y = \emptyset$. 
%         \end{tablenotes}
%     \end{threeparttable}
% \end{table}

==> s_dl_sat_table.tex <==
%!TEX root = lpmln_isets.tex

% \begin{table}
%     \centering
%     \caption{Relationships among SE-interpretations, rule $r$, and rule $\sdel{r}$ (Part I)}
%     \label{tab:single-del-sat}
%    \begin{tabular}{lccc}
%         \hline
%         $\#$ & Rule Types & $(X, Y) \models r$ & $(X, Y) \not\models r$  \\
%         \hline
%         1. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
%         2. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
%         3. & $\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $*$ & \textemdash \\  \hline
%         4. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
%         5. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\ \hline
%         6. & Others & $(X, Y) \models \sdel{r}$ & \textemdash  \\ 
%         \hline
%         \end{tabular}
% \end{table}

% \begin{table}
%     \centering
%     \caption{Relationships among SE-interpretations, rule $r$, and rule $\sdel{r}$ (Part II)}
%     \label{tab:single-del-sat-2}
%     \begin{tabular}{lccccc}
%         \hline
%         $\#$ & Rule Types & $\seinthalfadd{X}{Y} \models r$ & $\seinthalfadd{X}{Y} \not\models r$  & $\seintadd{X}{Y} \models r$ & $\seintadd{X}{Y} \not\models r$  \\
%         \hline
%         1. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
%         2. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $*$ & $*$ & \textemdash \\  \hline
%         3. & $\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $*$ & \textemdash & $(X, Y) \models \sdel{r}$ &  $(X, Y) \not\models \sdel{r}$ \\  \hline
%         4. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $*$ &  \textemdash & $*$ & \textemdash \\  \hline
%         5. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $*$ &  \textemdash & $*$ & \textemdash \\ \hline
%         6. & Others & $(X, Y) \models \sdel{r}$ & \textemdash & $(X, Y) \models \sdel{r}$ & \textemdash  \\ 
%         \hline
%         \end{tabular}

% \end{table}



\begin{table}
    \centering
    \caption{Relationships among SE-interpretations, rule $r$, and rule $\sdel{r}$ (Part I)}
    \label{tab:single-del-sat}
    \begin{threeparttable}
    \begin{tabular}{lccc}
        \hline
        $\#$ & Rule Types & $(X, Y) \models r$ & $(X, Y) \not\models r$  \\
        \hline
        1. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
        2. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
        3. & $\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $*$ & \textemdash \\  \hline
        4. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
        5. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\ \hline
        6. & Others & $(X, Y) \models \sdel{r}$ & \textemdash  \\ 
        \hline
        \end{tabular}

        \begin{tablenotes}
            \item The notation ``$*$'' means $(X, Y) ~\models~  \sdel{r}$ or $(X, Y) ~\not\models~  \sdel{r}$, and ``\textemdash'' means the case does not exist. 
        \end{tablenotes}
    \end{threeparttable}
\end{table}

\begin{table}
    \centering
    \caption{Relationships among SE-interpretations, rule $r$, and rule $\sdel{r}$ (Part II)}
    \label{tab:single-del-sat-2}
    \begin{threeparttable}
    \begin{tabular}{lccccc}
        \hline
        $\#$ & Rule Types & $\seinthalfadd{X}{Y} \models r$ & $\seinthalfadd{X}{Y} \not\models r$  & $\seintadd{X}{Y} \models r$ & $\seintadd{X}{Y} \not\models r$  \\
        \hline
        1. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ & $(X, Y) ~\models~  \sdel{r}$ & $(X, Y) ~\not\models~  \sdel{r}$ \\  \hline
        2. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $(X, Y) ~\models~  \sdel{r}$ & $*$ & $*$ & \textemdash \\  \hline
        3. & $\setdj{I}{\hr{r}}$, $\setsubeq{I}{\pbr{r}}$, $\setdj{I}{\nbr{r}}$ & $*$ & \textemdash & $(X, Y) \models \sdel{r}$ &  $(X, Y) \not\models \sdel{r}$ \\  \hline
        4. & $\setdj{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $*$ &  \textemdash & $*$ & \textemdash \\  \hline
        5. & $\setsubeq{I}{\hr{r}}$, $\setdj{I}{\pbr{r}}$, $\setsubeq{I}{\nbr{r}}$ & $*$ &  \textemdash & $*$ & \textemdash \\ \hline
        6. & Others & $(X, Y) \models \sdel{r}$ & \textemdash & $(X, Y) \models \sdel{r}$ & \textemdash  \\ 
        \hline
        \end{tabular}

        \begin{tablenotes}
            \item The notation ``$*$'' means $(X, Y) ~\models~  \sdel{r}$ or $(X, Y) ~\not\models~  \sdel{r}$, and  ``\textemdash'' means the case does not exist. 
        \end{tablenotes}
    \end{threeparttable}
\end{table}


==> todo.tex <==
%!TEX root = lpmln_qsr_se.tex

\section*{TODO}

Papers in ICLP reviews:
\begin{itemize}
    \item Ka-Shu Wong: Sound and Complete Inference Rules for SE-Consequence. J. Artif. Intell. Res. 31: 205-216 (2008)
    \item [Pearce 96] David Pearce, A New Logical Characterisation of Stable Models and Answer Sets, Non-Monotonic Extensions of Logic Programming, NMELP '96, LNCS 1216, pp. 57-70, 1996.
    \item [Ferraris et al. 07] Paolo Ferraris, Joohyung Lee, Vladimir Lifschitz: A New Perspective on Stable Models. IJCAI 2007: 372-379
    \item [Lifschitz et al 99] Vladimir Lifschitz, Lappoon R. Tang, Hudson Turner: Nested Expressions in Logic Programs. Ann. Math. Artif. Intell. 25(3-4): 369-389 (1999)
\end{itemize}


Ideas:
\begin{itemize}
    \item how to construct a pair of strongly equivalent logic programs from a known pair of programs. 
    \item LPOD strong equivalence
    \item forgetting under strong equivalence closely relates to single deletion operation (HT-forgetting), 
        (Wang Yisong et al., 2012, Forgetting in Logic Programs under Strong Equivalence)
    \item the definition of HT-forgetting is similar to the property of single deletion operation (Lemma)
\end{itemize}
